PersonaTwin: A Multi-Tier Prompt Conditioning Framework for Generating and Evaluating Personalized Digital Twins

While large language models (LLMs) afford new possibilities for user modeling and approximation of human behaviors, they often fail to capture the multidimensional nuances of individual users. In this work, we introduce PersonaTwin, a multi-tier prompt conditioning framework that builds adaptive digital twins by integrating demographic, behavioral, and psychometric data. Using a comprehensive data set in the healthcare context of more than 8,500 individuals, we systematically benchmark PersonaTwin against standard LLM outputs, and our rigorous evaluation unites state-of-the-art text similarity metrics with dedicated demographic parity assessments, ensuring that generated responses remain accurate and unbiased. Experimental results show that our framework produces simulation fidelity on par with oracle settings. Moreover, downstream models trained on persona-twins approximate models trained on individuals in terms of prediction and fairness metrics across both GPT-4o-based and Llama-based models. Together, these findings underscore the potential for LLM digital twin-based approaches in producing realistic and emotionally nuanced user simulations, offering a powerful tool for personalized digital user modeling and behavior analysis.

==> sections/Acknowledgements.tex <==

We would like to express our gratitude to the research team and student assistants who contributed to the data collection and processing phases of this study. Their dedicated efforts in annotating, cleaning, and managing the 8{,}500-participant psychometric dataset were instrumental to the success of \name. We also extend our thanks to the anonymous reviewers for their constructive feedback, which helped refine both our methodology and experimental design. We wish that this work will inspire continued innovation in fair and personalized healthcare technologies. Finally, we gratefully acknowledge the financial and institutional support provided by our respective universities and funding agencies, without which this work would not have been possible.

